Early Detection for Optimal-Latency Communications in Multi-Hop Links

Modern wireless machine-to-machine-type communications aim to provide both ultra reliability and low latency, stringent requirements that appear to be mutually exclusive. From the noisy channel coding theorem, we know that reliable communications mandate transmission rates that are lower than the channel capacity. To guarantee arbitrarily-low error probability, this implies the use of messages whose lengths tend to infinity. However, long messages are not suitable for low-latency communications. In this paper, we propose an early-detection scheme for wireless communications under a finite-blocklength regime that employs a sequential-test technique to reduce latency while maintaining reliability. We prove that our scheme leads to an average detection time smaller than the symbol duration. Furthermore, in multi-hop low-traffic or continuous-transmission links, we show that our scheme can reliably detect symbols before the end of their transmission, significantly reducing the latency, while keeping the error probability below a predefined threshold.

==> figures/res_multi_hop_Nbhops.tex <==
\definecolor{darkgreen}{RGB}{0, 128, 0}

\begin{tikzpicture}

  \pgfplotsset{
    grid style = {
      dash pattern = on 0.05mm off 1mm,
      line cap = round,
      black,
      line width = 0.5pt
    },
    title style = {font=\fontsize{7pt}{7.2}\selectfont},
    label style = {font=\fontsize{8pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }

  \begin{semilogyaxis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    grid=major,
    % xmin=0, xmax=10000,
    % xtick={0,2000,...,10000},
    xmin=0, xmax=2000,
    xtick={0,200,...,10000},
    scaled x ticks=false,
    xlabel={Information blocksize (bits)},
    xlabel style={yshift=0.6em},%
    %ymin=4e1, ymax=1e5,
    ymin=4e1, ymax=2e4,
    ylabel={\shortstack{Achievable average latency\\(normalized symbols)}},
    ylabel style={yshift=-1.0em},
    legend pos={south east},
    legend style={
      anchor={south east},
      cells={anchor=west},
      column sep=0mm,
      row sep=-0.5mm,
      font=\fontsize{7pt}{7.2}\selectfont,
      mark size=2.0pt,
      mark options=solid
    },
    mark size=2.0pt,
    mark options=solid,
    every axis plot/.append style={thick},
    ]
    \addplot [color=blue, mark=diamond]
    table[row sep=crcr]{%
      23.1503900471334	83.4307880163617\\
      36.5309192178481	107.225458187809\\
      50.5874933582085	133.769914066127\\
      111.045599870647	251.572346244755\\
      363.062438432575	791.163267498115\\
      540.504067169971	1200.74900623423\\
      813.386280380287	1854.20534233259\\
      1278.51454071799	3013.66479662094\\
      1751.32858902622	4206.82254784194\\
      4657.00863228216	11858.9926307341\\
      6624.37819201648	17314.8440163723\\
      9596.91320614996	25431.9878727799\\
      10591.6684799872	28170.2917458666\\
      14584.0821747206	39476.8562931377\\
      19595.7394514085	53312.5012332854\\
    };
    \addlegendentry{$h = 2$}

    \addplot [color=red, mark=x]
    table[row sep=crcr]{%
      23.1503900471334	125.732857715429\\
      36.5309192178481	162.853720661497\\
      50.5874933582085	201.749814462295\\
      111.045599870647	375.967444383855\\
      363.062438432575	1194.94604933422\\
      540.504067169971	1804.1197595195\\
      813.386280380287	2788.03889422549\\
      1278.51454071799	4494.83859935021\\
      1751.32858902622	6329.07211740052\\
      4657.00863228216	17883.3758511813\\
      6624.37819201648	25899.0312920143\\
      9596.91320614996	38148.503248216\\
      10591.6684799872	42247.2253675449\\
      14584.0821747206	59058.0554935254\\
      19595.7394514085	79929.2050952805\\
    };
    \addlegendentry{$h = 3$}

    \addplot [color=darkgreen, mark=o]
    table[row sep=crcr]{%
      23.1503900471334	166.664221237377\\
      36.5309192178481	215.904214090672\\
      50.5874933582085	268.545368358984\\
      111.045599870647	503.432768695313\\
      363.062438432575	1587.83834313842\\
      540.504067169971	2407.72255130518\\
      813.386280380287	3720.97643900591\\
      1278.51454071799	6034.18420267484\\
      1751.32858902622	8456.77660580464\\
      4657.00863228216	23892.0617424019\\
      6624.37819201648	34442.1093181195\\
      9596.91320614996	50954.8809169309\\
      10591.6684799872	56323.2921534788\\
      14584.0821747206	78659.096234874\\
      19595.7394514085	106943.307709814\\
    };
    \addlegendentry{$h = 4$}

    \addplot [color=black, mark=+]
    table[row sep=crcr]{%
      23.1503900471334	207.669474399173\\
      36.5309192178481	270.797257160401\\
      50.5874933582085	333.842594972725\\
      111.045599870647	629.067287847645\\
      363.062438432575	1978.41597116058\\
      540.504067169971	3001.66844730001\\
      813.386280380287	4649.9821975024\\
      1278.51454071799	7516.57543839284\\
      1751.32858902622	10573.7578762767\\
      4657.00863228216	29908.9630487359\\
      6624.37819201648	43207.1317691071\\
      9596.91320614996	63545.3614733283\\
      10591.6684799872	70756.5440074065\\
      14584.0821747206	98113.7029003423\\
      19595.7394514085	133401.412588762\\
    };
    \addlegendentry{$h = 5$}

  \end{semilogyaxis}
\end{tikzpicture}%

